Crowd Density Forecasting by Modeling Patch-based Dynamics

Forecasting human activities observed in videos is a long-standing challenge in computer vision, which leads to various real-world applications such as mobile robots, autonomous driving, and assistive systems. In this work, we present a new visual forecasting task called crowd density forecasting. Given a video of a crowd captured by a surveillance camera, our goal is to predict how that crowd will move in future frames. To address this task, we have developed the patch-based density forecasting network (PDFN), which enables forecasting over a sequence of crowd density maps describing how crowded each location is in each video frame. PDFN represents a crowd density map based on spatially overlapping patches and learns density dynamics patch-wise in a compact latent space. This enables us to model diverse and complex crowd density dynamics efficiently, even when the input video involves a variable number of crowds that each move independently. Experimental results with several public datasets demonstrate the effectiveness of our approach compared with state-of-the-art forecasting methods.

==> related_work.tex <==

The task of crowd density forecasting can be encompassed by visual forecasting that has been recognized as a long-standing challenge in computer vision. Below, we briefly review some recent work mainly presented recently.

\paragraph{Trajectory Forecasting in Computer Vision.}
Visual forecasting of human activities has widely been studied but remains a challenging problem in computer vision. In particular, much work has been done recently on trajectory forecasting, \ie, predicting a trajectory of how individual targets will move, with the rapid development of temporal modeling based on deep recurrent networks and imitation learning (\eg, \cite{Kitani2012}; see \cite{rudenko2019human} for a recent extensive survey). One key technical challenge, which is also closely related to our work, is how to forecast the trajectories of pedestrians interacting with each other in a group. Major approaches in this vein include social force modeling~\cite{Dirk1995,mehran2009abnormal}, multi-agent frameworks~\cite{le2017coordinated,ma2017forecasting,rhinehart2019precog,Zhao_2019_CVPR}, pooling states among multiple recurrent models~\cite{Alahi_2016_CVPR,Choi_2019_ICCV,Gupta_2018_CVPR,Lee_2017_CVPR,sadeghian2019sophie,Xu_2018_CVPR,Zhang_2019_CVPR}, and interaction modeling via graph neural networks~\cite{Ivanovic_2019_ICCV,vemula2018social}. However, all these works assume that accurate pedestrian trajectories are given both in training and testing. This is not always a realistic assumption when one wants to forecast the behaviors of a crowd because a large number of people would appear very small in each video frame and come with significant occlusions, making it difficult to detect and track them reliably. Our work resolves this issue by taking sequences of crowd density maps as inputs and outputs instead.

\paragraph{Other Relevant Forecasting Tasks.} 
There is also some work tackling a similar forecasting task in other research domains such as robotics~\cite{Bera_2017_IROS,Kretzschmar_2014_ICRA,Luber_2010_ICRA,Trautman_2015_IJRR}, intelligent vehicles~\cite{altche2017lstm,Chandra_2019_CVPR,houenou2013vehicle,Jain_2019_CoRL,Lee_2017_CVPR,Thiede_2019_ICCV,rhinehart2018r2p2,rhinehart2019precog}, and geo-spatial data analysis~\cite{zhou2014recognizing}. For example, recent work proposed a method that took auto-camera videos and LiDAR data as input to forecast vehicle trajectories~\cite{Chang_2019_CVPR,luo2018fast}. While such additional inputs would improve the crowd density forecasting ability of our approach, we limit our study to the use of a single surveillance video. \cite{Zhang_2017_AAAI,Zonoozi_2018_IJCAI} have attempted to enable city-scale forecasting of vehicle motion by making use of GPS histories. Similar to our work, they learn crowd dynamics with a convolutional neural network. However, their models focus only on a specific scenario in which training and testing videos are captured in the same scene. In contrast, our approach can work on a variety of complex crowd density dynamics due to its novel patch-based representation.

\paragraph{Crowd Density Estimation.}
Lastly, our work is also relevant to crowd density estimation, which is another popular computer vision task aiming to detect and count crowds in still images or videos.  Despite a huge amount of prior work (see \cite{kang2018beyond,sindagi2018survey,zitouni2016advances} for extensive surveys), attempts on video-based crowd density estimation are relatively limited \cite{fang2019locality,liu2019geometric,xingjian2015convolutional,zhang2017fcn}, and their main focus lies in how to leverage temporal continuities for improving density estimation, rather than how to forecast future crowdedness.

